Automating the Detection of Code Vulnerabilities by Analyzing GitHub Issues

In today's digital landscape, the importance of timely and accurate vulnerability detection has significantly increased. This paper presents a novel approach that leverages transformer-based models and machine learning techniques to automate the identification of software vulnerabilities by analyzing GitHub issues. We introduce a new dataset specifically designed for classifying GitHub issues relevant to vulnerability detection. We then examine various classification techniques to determine their effectiveness. The results demonstrate the potential of this approach for real-world application in early vulnerability detection, which could substantially reduce the window of exploitation for software vulnerabilities. This research makes a key contribution to the field by providing a scalable and computationally efficient framework for automated detection, enabling the prevention of compromised software usage before official notifications. This work has the potential to enhance the security of open-source software ecosystems.

==> sections/666-new-experiment.tex <==
\section{Model Performance on Post-Knowledge Cutoff Vulnerabilities}
\label{sec:post_cutoff_analysis}

\todo[inline]{we merge this section with last section}

In this analysis, we evaluate, to the extent possible, the performance of our model on the portion of the dataset that includes issues and vulnerabilities that arose after the knowledge cutoff date of the GPT-4o-mini model, specifically after October 2023\cite{noauthor_openai_nodate}. As discussed in detail in the section \textit{Threats to Validity}, we lack visibility into the composition of the training set used for the LLM. Therefore, the only viable method to ensure that our solutions do not suffer from overfitting is to evaluate the model using data generated after the cutoff.
\\\\
As explained in the following section, it was not feasible to use such a dataset for all the experimentation since the model employed is relatively new, and there are a few vulnerabilities that have been reported after its cutoff date. Consequently, the available dataset for this kind of analysis is quite limited.
\\\\
Specifically, within our test set, 29 tracking issues are post-cutoff, and 672 normal issues. Nonetheless, this evaluation provides critical insights into the model's ability to generalize to new, unseen vulnerabilities, offering a preliminary indication of its robustness and applicability in real-world scenarios.

\begin{table}[ht!]
\label{tab:report_cutoff}
\caption[Classification Report]{Detailed classification metrics for combined methodology on post knowledge cutoff test set} 
\vspace{1em}
\centering
\begin{tabular}{l *{4}{S[table-format=2.2]}}
{} & \multicolumn{4}{c}{Classification Metrics} \\
\cmidrule{2-5}
Class & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1-Score} & \multicolumn{1}{c}{Support} \\
\midrule
0 & 0.99 & 0.95 & 0.97 & 672 \\
1  & 0.41 & 0.83 & 0.55 & 29 \\
\midrule
\textbf{Accuracy} & \multicolumn{4}{c}{0.94} \\
\end{tabular}
\end{table}

The support of the new dataset, defined as the number of occurrences of the class within the dataset, has significantly changed compared to the initial dataset. Consequently, the proportion of Class 1 has shifted from 19\% to 4\%. This change highlights the lower percentage of relevant issues within the new data sample, aligning more closely with a realistic scenario. This disparity between the distributions of the two datasets complicates the direct comparison of the results obtained in the previous sections.


\subsection{Descriptions similarity}

It is also crucial to examine the quality and relevance of the vulnerability descriptions generated by the LLM for post-knowledge cutoff issues.
\\

% \begin{figure}[!ht]
%   \begin{center}
%     \includegraphics[width=0.5\textwidth]{figures/cutoff_similarity.pdf}    
%   \end{center}
%   \caption{Distribution of similarity scores for descriptions generated by the few-shot model on the post-knowledge cutoff test set}
%   \label{fig:few-sim}
% \end{figure}

% \begin{table}[ht!]
% \caption{Similarity Scores for the Few-Shot Model}
% \label{tab:simi_few_shot}
% \vspace{1em}
% \centering
% \begin{tabular}{l *{1}{S[table-format=1.6]}}
% \toprule
% Metric & \multicolumn{1}{c}{Few-Shot} \\
% \midrule
% Mean Similarity & 0.756 \\
% Median Similarity & 0.775 \\
% \bottomrule
% \end{tabular}
% \end{table}

The similarity scores across different datasets suggest that the model effectively generalizes to new, unseen issues, reinforcing the reliability of the model. This consistency is promising and implies that the model's performance is robust and not limited to the initial training set.
